Unsupervised Out-of-Distribution Detection in Medical Imaging Using Multi-Exit Class Activation Maps and Feature Masking

Out-of-distribution (OOD) detection is essential for ensuring the reliability of deep learning models in medical imaging applications. This work is motivated by the observation that class activation maps (CAMs) for in-distribution (ID) data typically emphasize regions that are highly relevant to the model's predictions, whereas OOD data often lacks such focused activations. By masking input images with inverted CAMs, the feature representations of ID data undergo more substantial changes compared to those of OOD data, offering a robust criterion for differentiation. In this paper, we introduce a novel unsupervised OOD detection framework, Multi-Exit Class Activation Map (MECAM), which leverages multi-exit CAMs and feature masking. By utilizing mult-exit networks that combine CAMs from varying resolutions and depths, our method captures both global and local feature representations, thereby enhancing the robustness of OOD detection. We evaluate MECAM on multiple ID datasets, including ISIC19 and PathMNIST, and test its performance against three medical OOD datasets, RSNA Pneumonia, COVID-19, and HeadCT, and one natural image OOD dataset, iSUN. Comprehensive comparisons with state-of-the-art OOD detection methods validate the effectiveness of our approach. Our findings emphasize the potential of multi-exit networks and feature masking for advancing unsupervised OOD detection in medical imaging, paving the way for more reliable and interpretable models in clinical practice.

==> Table/ablation_weighted_sum.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Ablation study on the OOD detection performance of aggregating CAM from different exits using average or weighted-sum (proposed) in the proposed model with the PathMNIST dataset using ResNet-50.}
% \setlength{\tabcolsep}{1pt}
\label{Table:ablation_weighted_sum}
\begin{tabular}{c|cccccccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{8}{c}{OOD} \\ \cline{2-9} 
 & \multicolumn{2}{c}{RSNA} & \multicolumn{2}{c}{COVID-19} & \multicolumn{2}{c}{HeadCT} & \multicolumn{2}{c}{iSUN} \\ \cline{2-9} 
 & FPR95 $\downarrow$ & AUC $\uparrow$ & FPR95 $\downarrow$ & AUC $\uparrow$ & FPR95 $\downarrow$ & AUC $\uparrow$ & FPR95 $\downarrow$ & AUC $\uparrow$ \\ \hline
Average & 00.43 & 99.66 & 03.85 & 98.98 & 06.00 & 98.65 & 05.11 & 98.35 \\
Weighted-sum & \textbf{00.30} & \textbf{99.69} & \textbf{02.80} & \textbf{99.06} & \textbf{03.50} & \textbf{98.88} & \textbf{04.29} & \textbf{98.45} \\ \hline
\end{tabular}
\end{table}
